Multicast Beamformer Design for MIMO Coded Caching Systems

Coded caching (CC) techniques have been shown to be conveniently applicable in multi-input multi-output (MIMO) systems. In a $K$-user network with spatial multiplexing gains of $L$ at the transmitter and $G$ at every receiver, if each user can cache a fraction $\gamma$ of the file library, a total number of $GK\gamma + L$ data streams can be served in parallel. In this paper, we focus on improving the finite-SNR performance of MIMO-CC systems. We first consider a MIMO-CC scheme that relies only on unicasting individual data streams, and then, introduce a decomposition strategy to design a new scheme that delivers the same data streams through multicasting of $G$ parallel codewords. We discuss how optimized beamformers could be designed for each scheme and use numerical simulations to compare their finite-SNR performance. It is shown that while both schemes serve the same number of streams, multicasting provides notable performance improvements. This is because, with multicasting, transmission vectors are built with fewer beamformers, leading to more efficient usage of available power resources.

==> 3UserExample_Prop.tex <==
\begin{exmp}
\label{exmp:proposed}
Consider the network in Example~\ref{exmp:wsa}. The idea is that instead of transmitting $\Bx([3])$ in~\eqref{eq:exmp_trans_wsa}, we transmit
\begin{equation*}
\begin{aligned}
    \hat{\Bx}([3]) = &(A_{23}^1 \oplus B_{13}^3) \Bw_{{\Sfs_2^1}{\Sfs_2^2}} + (B_{13}^1 \oplus C_{12}^3) \Bw_{{\Sfs_3^1}{\Sfs_3^2}} + \\
    &(C_{12}^1 \oplus A_{23}^3) \Bw_{{\Sfs_1^1}{\Sfs_1^2}} + (A_{23}^2 \oplus B_{13}^2) \Bw_{{\Sfs_1^1}{\Sfs_2^1}} + C_{12}^2 \Bw_{{\Sfs_3^1}} \; ,
\end{aligned}
\end{equation*}
which achieves the same DoF but with only five beamformers (instead of nine). Of course, now we need new feedback loops among the receiver chains, as shown in Figure~\ref{fig:receiver_Prop}. Let us consider the decoding process in user~1. This user has to start by decoding the first data stream ($A_{23}^1$) using the received signal
\begin{equation*}
\begin{aligned}
    \hat{y}_1^1([3]) = &(A_{23}^1 \oplus B_{13}^3) \Bh_{1,1}^H \Bw_{{\Sfs_2^1}{\Sfs_2^2}} + (C_{12}^1 \oplus A_{23}^3) \Bh_{1,1}^H \Bw_{{\Sfs_1^1}{\Sfs_1^2}} + \\
    &(A_{23}^2 \oplus B_{13}^2) \Bh_{1,1}^H\Bw_{{\Sfs_1^1}{\Sfs_2^1}} + I_c + z_1^1([3]) 
\end{aligned}
\end{equation*}
%
%We achieve the same DoF, but with a higher finite-SNR rate. The key idea is to use an ordering in decoding the streams. Here, the ordering is to start from the smallest index and move to the largest one.
%The first stream signal at user 1 can be written as
%\begin{equation}
%\begin{aligned}
%    \hat{y}_1^1(\CS) = &(A_{23}^1 \oplus B_{13}^3) \Bh_{1,1}^H \Bw_{{_2^1}{_2^2}} + (C_{12}^1 \oplus A_{23}^3) \Bh_{1,1}^H \Bw_{{_1^1}{_1^2}} + 
%    \\& (A_{23}^2 \oplus B_{13}^2) \Bh_{1,1}^H\Bw_{{_1^1}{_2^1}} + I_c + z_1^1(\CS) 
%\end{aligned}
%\end{equation}
where the interference term $I_c = (B_{13}^1 \oplus C_{12}^3) \Bh_{1,1}^H\Bw_{{\Sfs_3^1}{\Sfs_3^2}} + C_{12}^2 \Bh_{1,1}^H\Bw_{{\Sfs_3^1}}$ can be reconstructed and removed using the cache contents of user~1. The codeword $A_{23}^1 \oplus B_{13}^3$ can then be decoded with the rate
    \begin{equation*}
        \hat{r}_1^1 \le \log(1+\frac{|\Bh_{1,1}^H \Bw_{{\Sfs_2^1} {\Sfs_2^2}}|^2}{|\Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^2}}|^2 + |\Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_2^1}}|^2 + N_0}) \; ,
    \end{equation*}
and after that, the requested term $A_{23}^1$ can be extracted by removing $B_{13}^3$ (which is available in the cache). After decoding $A_{23}^1$, user~1 can proceed with decoding the second stream ($A_{23}^2$), using the received signal ...

%Now, let us consider the second stream at user 1, which is ...


%We achieve the same DoF, but with a higher finite-SNR rate. Beamformers are calculated as ....

%The reason for the higher data rate is the fewer beamforming vectors, which results in higher average power per beamformer. This is more effective in the finite-SNR regime as we are power-limited in this regime. 

%The receiver structure for this receiver structure is shown in Figure~\ref{fig:receiver_Prop}.


\end{exmp}

==> 3UserExample_WSA.tex <==
\begin{exmp}
\label{exmp:wsa}
    Consider a small network with $K=3$ users, coded caching gain of $t=2$, $L=3$ antennas at the transmitter, and $G=3$ antennas at each receiver. As $K = t+\eta$, we need only a single transmission to deliver the missing data. Denoting the files requested by users 1-3 by $A$, $B$, and $C$, this transmission vector is built as
    %each with $G=3$ receiver antennas and a cache memory large enough to store $\gamma=\frac{2}{3}$ of the whole library (i.e., $t=2$). The users request data from a transmitter with $L=3$ antennas. Assume the content placement is done following the MS scheme, and in the delivery phase, users 1-6 request files $A$, $B$, ..., $F$, respectively. Using the MIMO CC extension in~\cite{salehi2021MIMO}, each transmission vector delivers data to $t+\frac{L}{G} = 3$ users, while each user receives $G=3$ streams simultaneously (i.e., the DoF is $Gt+L=9$). Considering the transmission vector for the set of users $\CS = \{1,2,3\}$, we have
    \begin{equation}
    \label{eq:exmp_trans_wsa}
        \begin{aligned}
            \Bx([3]) &= A_{23}^1 \Bw_{{\Sfs_1^2} {\Sfs_1^3}} + B_{13}^1 \Bw_{{\Sfs_2^2} {\Sfs_2^3}} + C_{12}^1 \Bw_{{\Sfs_3^2} {\Sfs_3^3}} \\ &+
            A_{23}^2 \Bw_{{\Sfs_1^1} {\Sfs_1^3}} + B_{13}^2 \Bw_{{\Sfs_2^1} {\Sfs_2^3}} + C_{12}^2 \Bw_{{\Sfs_3^1} {\Sfs_3^3}} \\ &+
            A_{23}^3 \Bw_{{\Sfs_1^1} {\Sfs_1^2}} + B_{13}^3 \Bw_{{\Sfs_2^1} {\Sfs_2^2}} + C_{12}^3 \Bw_{{\Sfs_3^1} {\Sfs_3^2}} \; .
        \end{aligned}
    \end{equation}
    Let us consider the decoding process for the first data stream for user~1, i.e., $A_{23}^1$. Using ..., we have
    %Now, using ..., the first stream signal at user 1 is
    \begin{equation*}
        \begin{aligned}
            y_1^1([3]) = &\Bh_{1,1}^H \Bx([3]) + z_1^1([3]) = A_{23}^1 \Bh_{1,1}^H \Bw_{{\Sfs_1^2} {\Sfs_1^3}} +\\
            &A_{23}^2 \Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^3}} + A_{23}^3 \Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^2}} +
            I_c + z_1^1([3]) \; ,
        \end{aligned}
    \end{equation*}
    where the interference term $I_c = \Bh_{1,1}^H(B_{13}^1 \Bw_{{\Sfs_2^2} {\Sfs_2^3}} + C_{12}^1 \Bw_{{\Sfs_3^2} {\Sfs_3^3}} + B_{13}^2 \Bw_{{\Sfs_2^1} {\Sfs_2^3}} + C_{12}^2 \Bw_{{\Sfs_3^1} {\Sfs_3^3}} + B_{13}^3 \Bw_{{\Sfs_2^1} {\Sfs_2^2}} + C_{12}^3 \Bw_{{\Sfs_3^1} {\Sfs_3^2}})$ can be fully reconstructed and removed using the cache contents of user~1.\footnote{In this paper, we assume that equivalent channel multipliers (i.e., $\Bh_{k,g}^H \Bw_{\CR}$) can be estimated at the receivers, e.g., using downlink precoded pilots.} So, the rate region for decoding $A_{23}^1$ at user~1 is given by
    %\begin{equation}
    %    \begin{aligned}
     %       y_1^1 (\CS) = &A_{23}^1 \Bh_{1,1}^H \Bw_{{\Sfs_1^2} {\Sfs_1^3}} + \underline{B_{13}^1 \Bh_{1,1}^H \Bw_{{_2^2} {_2^3}}} + \underline{C_{12}^1 \Bh_{1,1}^H \Bw_{{_3^2} {_3^3}}} +  \\
     %       &A_{23}^2 \Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^3}} + \underline{B_{13}^2 \Bh_{1,1}^H \Bw_{{_2^1} {_2^3}}} + \underline{C_{12}^2 \Bh_{1,1}^H \Bw_{{_3^1} {_3^3}}} +  \\
     %       &A_{23}^3 \Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^2}} + \underline{B_{13}^3 \Bh_{1,1}^H \Bw_{{_2^1} {_2^2}}} + \underline{C_{12}^3 \Bh_{1,1}^H \Bw_{{_3^1} {_3^2}}} + z_1^1(\CS)
    %    \end{aligned}    
    %\end{equation}
    %Following ..., we want to take out the data term $A_{23}^1$ from this stream. However, the underlined terms in ... are available in the cache memory of user 1, and their interference can be reconstructed and removed from $y_1^1(\CS)$. Hence, for the decoding rate of this data term, we will have
    \begin{equation*}
        r_1^1 \le \log(1+\frac{|\Bh_{1,1}^H \Bw_{{\Sfs_1^2} {\Sfs_1^3}}|^2}{|\Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^3}}|^2 + |\Bh_{1,1}^H \Bw_{{\Sfs_1^1} {\Sfs_1^2}}|^2 + N_0}) \; ,
    \end{equation*}
    and the rate regions for decoding other terms can also be calculated accordingly.
    Finally, the rate optimization problem can be written as
    \begin{equation*}
        \begin{aligned}
            \max_{k,g \in [3]} r_k^g \qquad s.t. \sum_{k,g,h \in [3], g \neq h} {|\Bw_{\Sfs_k^g \Sfs_k^h}|^2} \le P_T
        \end{aligned}
    \end{equation*}
    Of course, the result of this optimization problem depends also on receive beamformers $\Bu_{k,g}$, which should be designed at the same time as transmit beamformers using alternate optimizations. Figure~\ref{fig:receiver_WSA} represents the receiver structure for this example. Note that all data streams can be decoded in parallel.
    %Going through all streams for all users, the beamformer optimization problem could be written as ...
    %The receiver structure for this example is shown in Figure~\ref{fig:receiver_WSA}.

    \begin{figure}
    %\begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[height = 5cm]{Figs/Receiver_WSA.png}
        %\vspace{5pt}
    %\end{subfigure}
    \caption{Add caption}
    \label{fig:receiver_WSA}
    \end{figure}
\end{exmp}

%\subsection{Coded Caching with Signal-level Interference Cancellation}
%\input{SigLevelIntCan.tex}

%\subsection{The baseline MIMO CC scheme}
%\input{MIMOCC.tex}

==> AddingXOR.tex <==
In this section, we show how MMSE-SIC based receiver processing, proper decoding order of the data streams and multicast beamformer design...  can considerably improve the finite-SNR performance of \ac{MIMO}-CC schemes. Instead of using the unicast beamformer desing and linear MMSE receiver structure in Figure~\ref{fig:receiver_WSA}, we use the one shown in Figure~\ref{fig:receiver_Prop} where the output of every decoder stage is used to remove part of the interference in the next stage(s). %Using such a feedback structure in \ac{MIMO} setups is not new and has been investigated thoroughly in the literature~[REFS]. 
The MMSE-SIC structure allows us to .... 
However, in the context of \ac{MIMO}-CC schemes, this feedback structure could be more effective as it enables (re)introducing XOR codewords and hence, improving the multicasting gain~\cite{salehi2019subpacketization},[ASILOMAR]. Next, we first explore the idea in Example~\ref{exmp:proposed_k2} and then present the structural design for the general case.

    %\begin{figure}
    %%\begin{subfigure}{\columnwidth}
    %    \centering
    %    \includegraphics[height = 5cm]{Figs/Receiver_Prop.png}
    %    %\vspace{5pt}
    %%\end{subfigure}
    %\caption{Add caption}
    %\label{fig:receiver_Prop}
    %\end{figure}

%Using the MIMO coded caching scheme in~\cite{salehi2021MIMO}, the number of simultaneous data streams (and hence, the DoF) can be improved considerably. However, as shown in Example~\ref{exmp:wsa}, this scheme requires decoupling every XOR codeword and sending each data stream with a separate beamformer. From~\cite{salehi2019subpacketization},[ASILOMAR], we know that such decoupling of XOR codewords would degrade the performance in the finite-SNR regime as the available transmit power is split over more beamformers, and the rate is power-limited in finite-SNR. In this paper, we show that by enabling feedback loops among the receiver chains, it is possible to reintroduce XOR codewords in MIMO coded caching and reduce the number of required beamformers by a factor of two. We first review the process in Example~\ref{exmp:proposed}, and then, introduce the general algorithm.

\begin{exmp}
    \label{exmp:proposed_k2}
    Consider the network in Example~\ref{exmp:wsa_k2}. We show that with a proper decoding order we can deliver the same four data streams as in $\Bx([2])$ using
    \begin{equation}
        \hat{\Bx}([2]) = (A_2^1 \oplus B_1^2) \hat{\Bw}_{\Sfs_2^1} + (A_2^2 \oplus B_1^1) \hat{\Bw}_{\Sfs_1^1} \; ,
    \end{equation}
    which requires half the number of beamforming vectors compared with~\eqref{eq:trans_vector_wsa_exmp}. To do so, at the receivers of both users~1 and~2 we should start by decoding the first data stream, and subtract its interference from the received signal before decoding the second data stream. Let us consider the process in user~1. The received signal for the first stream is
    \begin{equation*}
    \begin{aligned}
        \hat{y}_1^1([2]) &= \Bh_{1,1}^H \hat{\Bx}([2]) \\
        &= (A_2^1 \oplus B_1^2) \Bh_{1,1}^H\hat{\Bw}_{\Sfs_2^1} + (A_2^2 \oplus B_1^1) \Bh_{1,1}^H\hat{\Bw}_{\Sfs_1^1} + z_1^1 \; ,
    \end{aligned}
    \end{equation*}
    and the codeword $(A_2^1 \oplus B_1^2)$ can be decoded with the rate
    \begin{equation*}
        \hat{r}_1^1 \le \log \Big( 1 + \frac{|\Bh_{1,1}^H \hat{\Bw}_{\Sfs_2^1}|^2}{|\Bh_{1,1}^H \hat{\Bw}_{\Sfs_1^1}|^2 + N_0} \Big) \; .
    \end{equation*}
    Finally, the data term $A_2^1$ can be extracted by removing $B_1^2$, which is available in the cache memory of user~1. Next, user~1 has to decode $A_2^2$ using the received signal
    \begin{equation*}
    \begin{aligned}
        \hat{y}_1^2([2]) = (A_2^1 \oplus B_1^2) \Bh_{1,2}^H\hat{\Bw}_{\Sfs_2^1} + (A_2^2 \oplus B_1^1) \Bh_{1,2}^H\hat{\Bw}_{\Sfs_1^1} + z_1^2 \; .
    \end{aligned}
    \end{equation*}
    However, now that $A_2^1$ is already decoded and $B_1^2$ is available in the cache, user~1 can reconstruct and remove the interference term $(A_2^1 \oplus B_1^2) \Bh_{1,2}^H\hat{\Bw}_{\Sfs_2^1}$ from the received signal, and decode the codeword $(A_2^2 \oplus B_1^1)$ with data rate
    \begin{equation*}
        \hat{r}_1^2 \le \log \Big( 1 + \frac{|\Bh_{1,2}^H \hat{\Bw}_{\Sfs_1^1}|^2}{N_0} \Big). 
    \end{equation*}
    Following the same procedure for user~2, the symmetric rate can be calculated by solving
    \begin{equation}
    \label{eq:sym_rate_prop_exmp}
        \begin{aligned}
            \hat{r} = &\max \min_{k,g \in [2]} \hat{r}_k^g \\
            s.t. \quad & \hat{r}_k^1 \le  \log \Big( 1 + \frac{|\Bh_{k,1}^H \hat{\Bw}_{\Sfs_{|k-2|+1}^1}|^2}{|\Bh_{k,1}^H \hat{\Bw}_{\Sfs_k^1}|^2 + N_0} \Big) , \;\; k \in [2] \\
            &\hat{r}_k^2 \le \log \Big( 1 + \frac{|\Bh_{k,2}^H \hat{\Bw}_{\Sfs_k^1|^2}}{N_0} \Big) , \;\; k \in [2] \; , \\
            &|\Bw_{\Sfs_1^1}|^2 + |\Bw_{\Sfs_2^1}|^2 \le P_T \; .
        \end{aligned}
    \end{equation}
    Comparing the optimization problems in~\eqref{eq:sym_rate_wsa_exmp} and~\eqref{eq:sym_rate_prop_exmp}, we expect $\hat{r} \le r$. This is because, with the proposed scheme, we need fewer beamformers, and the average power per beamformer increases. This results in an improved rate, especially in the finite-SNR regime. Note that the optimization problem in~\eqref{eq:sym_rate_prop_exmp} is also non-convex and requires successive interference cancellation and alternating optimization as in~\eqref{eq:sym_rate_wsa_exmp}.
\end{exmp}

In the general case, after decoding every data stream, its interference on other streams is reconstructed and removed before decoding them. This enables part of the interference that was previously suppressed by beamformers to be fully removed using the feedback loop. The result is more freedom in designing beamformers, which can be used also to build multicast codewords.

After using the feedback structure in Figure~\ref{fig:receiver_Prop}, data streams could be put into codewords in various ways. In this paper, we propose a straightforward algorithm that creates XOR codewords of size two, thus halving the number of required beamformers. To achieve this goal, we use a \textit{codeword guide} matrix $\BC$, which is a $G \times (t+1)$ matrix with integer elements. Every row in $\BC$ denotes a stream index and each column represents one of the users in a subset $\CT$ of users with $|\CT| = t+1$ (c.f.~(eq) in Section~\ref{section:sys_model}). The matrix $\BC$ is built using algorithm~\ref{alg:c_mat_build}. In a nutshell, the upper part of $\BC$ is filled up with consecutive integers and the lower half is a circular shift of the upper part by one unit to the right. If the number of rows is odd, in the middle row the consecutive numbering follows by repeating every integer two times. For example, if $t=1$ and $G=2$ (the parameters used in Examples ...), we have
\begin{equation}
    \BC =
    \begin{bmatrix}
        1 & 2 \\
        2 & 1
    \end{bmatrix} ,
\end{equation}
while if $t=4$ and $G=3$ we have
\begin{equation}
    \BC =
    \begin{bmatrix}
        1 & 2 & 3 & 4 & 5 \\
        6 & 6 & 7 & 7 & 8 \\
        5 & 1 & 2 & 3 & 4
    \end{bmatrix} .
\end{equation}

After building $\BC$, for every set of users $\CT$ appearing in a transmission vector, we can create codewords of elements having similar numbers in $\BC$. For example, ...

\begin{algorithm}
\caption{Build $\BC$}
\label{alg:c_mat_build}
\begin{algorithmic}[1]
    \State $c \gets 1$
    \For{$1 \le i \le \lfloor G/2 \rfloor$}
        \For{$1 \le j \le t+1$}
            \State $\BC[i,j] \gets c$
            \State $\BC[G-i+1,j \mod (t+1) +1] \gets c$
            \State $c \gets c+1$
        \EndFor 
    \EndFor
    \If{$G/2 \neq \lfloor G/2 \rfloor$}
        \For{$1 \le j \le \lfloor (t+1)/2 \rfloor$}
            \State $\BC[\lfloor G/2 \rfloor + 1, 2j-1] \gets c$
            \State $\BC[\lfloor G/2 \rfloor + 1, 2j] \gets c$
            \State $c \gets c+1$
        \EndFor
        \If{$(t+1)/2 \neq \lfloor (t+1)/2 \rfloor$}
            \State $\BC[\lfloor G/2 \rfloor + 1, t+1] \gets c$
        \EndIf
    \EndIf
\end{algorithmic}
\end{algorithm}

The rationale behind this codeword creation is that with the proposed decoding order (i.e., starting from the first data stream and moving down over the streams), the interference from the stream $i$ will be removed over all the streams $i+1$ to $G$ and does not need to be suppressed by its associated beamformer. Thus we have more freedom in beamformer design as we move up through the streams. This enables us to put higher index streams in the same codeword with the lower index ones.

%For the general case, the feedback loop enables the data terms in former stages to be treated as cache contents in the next stages, thus removing the necessity of removing their interference with beamformer vectors. This simplifies the constraints while designing beamformers, enabling the creation of XOR codewords. DISCUSS HOW THE $\CR$ SETS ARE REDUCED. In this paper, we use a circular structure to create XORs. Of course there exist many ways to do so.




==> Exmp_4Antenna.tex <==
\begin{exmp}
    Consider a network of $K=6$ users, each with $G=4$ antennas, that is served by a single transmitter with $L=4$ antennas. The users have cache memories, and the caching gain is $t=2$. Without MIMO CC techniques (i.e., by using receiver-side antennas just to have a better beamforming gain), we can serve $t+L=6$ users simultaneously, delivering one stream per user. However, with the proposed MIMO CC scheme, while we serve $t+\frac{L}{G}=3$ users per transmission, each user receives $G=4$ simultaneous streams. As a result, the DoF is increased from $6$ to $12$. Let us consider the transmission vector for users $1,2,3$, and assume the files requested by these three users are shown by $A,B,C$, respectively. Following the discussions in ..., this transmission vector is built as:
    \begin{equation}
        \begin{aligned}
            \Bx_{\CS = [3]} = &A_{23}^1 \Bw_{{_1^2} {_1^3} {_1^4}} + B_{13}^1 \Bw_{{_2^2} {_2^3} {_2^4}} + C_{12}^1 \Bw_{{_3^2} {_3^3} {_3^4}} +  \\
            &A_{23}^2 \Bw_{{_1^1} {_1^3} {_1^4}} + B_{13}^2 \Bw_{{_2^1} {_2^3} {_2^4}} + C_{12}^2 \Bw_{{_3^1} {_3^3} {_3^4}} +  \\
            &A_{23}^3 \Bw_{{_1^1} {_1^2} {_1^4}} + B_{13}^3 \Bw_{{_2^1} {_2^2} {_2^4}} + C_{12}^3 \Bw_{{_3^1} {_3^2} {_3^4}} +  \\
            &A_{23}^4 \Bw_{{_1^1} {_1^2} {_1^3}} + B_{13}^4 \Bw_{{_2^1} {_2^2} {_2^3}} + C_{12}^4 \Bw_{{_3^1} {_3^2} {_3^3}}
        \end{aligned}
    \end{equation}
    It can be easily seen that after transmitting $\Bx_{\CS=[3]}$, all the twelve data streams within it can be decoded simultaneously and interference-free. For example, for the first stream in user 1 (associated with the data term $A_{23}^1$), all the data terms for users 2 and 3 (i.e., $B_{13}^q$ and $C_{12}^q$, for $q \in [4]$) are available in the cache memory of user 1 and their interference can be constructed and removed from the received signal. Also, interference from other data terms for user 1 (i.e., $A_{23}^q$ for $q \in \{2,3,4\}$) is suppressed on the target data stream using the beamforming vectors (i.e., ${_1^1}$ is in the sub-index set of all the respective beamformers).

    Now, we argue that with proper decoding order, we can deliver the same twelve streams as in $\Bx_{\CS=[3]}$ using the following transmission vector:
    \begin{equation}
        \begin{aligned}
            &\hat{\Bx}_{\CS=[3]} =  \\
            &(A_{23}^1 \oplus B_{13}^4) \Bw_{{_2^1} {_2^2} {_2^3}} + (B_{13}^1 \oplus C_{12}^4) \Bw_{{_3^1} {_3^2} {_3^3}} + (C_{12}^1 \oplus A_{23}^4) \Bw_{{_1^1} {_1^2} {_1^3}} + \\
            &(A_{23}^2 \oplus B_{13}^3) \Bw_{{_1^1} {_2^1} {_2^2}} + (B_{13}^2 \oplus C_{12}^3) \Bw_{{_2^1} {_3^1} {_3^2}} + (C_{12}^2 \oplus A_{23}^3) \Bw_{{_3^1} {_1^1} {_1^2}}
        \end{aligned}
    \end{equation}
    The key is to decode data streams following their superscript index. Let us consider user one, for example. First, we need to decode the first data stream, i.e., $A_{23}^1$. For this stream, the interference terms $(B_{13}^1 \oplus C_{12}^4) \Bw_{{_3^1} {_3^2} {_3^3}}$ and $(B_{13}^2 \oplus C_{12}^3) \Bw_{{_2^1} {_3^1} {_3^2}}$ are removed using the cache contents, and the other three interference terms are suppressed with beamforming as ${_1^1}$ is in the subscript of the beamformers. Now, user one starts to decode the second data term, i.e., $A_{23}^2$. For this data term, again two interference terms are removed by the cache. However, only two interference terms out of the remaining three are removed by beamforming. But the key is that, after decoding $A_{23}^1$, the interference from the term $(A_{23}^1 \oplus B_{13}^4) \Bw_{{_2^1} {_2^2} {_2^3}}$ can also be reconstructed and removed (as $A_{23}^1$ is already decoded). Hence, $A_{23}^2$ can also be decoded interference-free. Similarly, $A_{23}^3$ and $A_{23}^4$ can also be decoded with proper ordering.
\end{exmp}

==> ExtAbstract.tex <==




%In this paper, we extend the applicability of coded caching to \ac{MIMO} communications with multi-antenna receivers. We show that \ac{MIMO} coded caching can be considered as an extension of the shared-cache setting studied in~\cite{parrinello2019fundamental,parrinello2020extending}. In shared-cache setups, a number of single-antenna users are aided by a smaller number of shared-cache nodes (which can be, e.g., helper nodes) while requesting data from a multi-antenna transmitting server. To extend this model to \ac{MIMO} coded caching, we can assume each shared-cache node represents a multi-antenna receiver, and each single-antenna user is replaced by an antenna element. Such an extension paves the way to using the optimality results in~\cite{parrinello2019fundamental,parrinello2020extending} to \ac{MIMO} coded caching. Specifically, in case all the users in a \ac{MIMO} setup have more than $G$ number of receiving antennas\footnote{$G$ represents the number of independent streams transmitted to each receiver.}, assuming large enough $L$, we get the interesting result that the coded caching gain $t$ can be multiplied by $G$, and a cumulative single-shot \ac{DoF} of $Gt+L$ becomes achievable.

%We also propose a new algorithm for creating \ac{MIMO} coded caching schemes, where we elevate baseline linear \ac{MISO} schemes already available in the literature to be applicable to \ac{MIMO} setups while achieving the increased \ac{DoF} of $Gt+L$. The elevation method is applicable when the number of dedicated streams to each receiver divides the number of transmit antennas (i.e., when $\eta := \frac{L}{G}$ is an integer), and achieves the full \ac{DoF} of $Gt+L$ if the baseline \ac{MISO} scheme supports the \ac{DoF} of $t+L$. This enables designing low-complexity, low-subpacketization \ac{MIMO} schemes with full \ac{DoF} using an appropriate \ac{MISO} scheme such as the one in~\cite{salehi2020lowcomplexity}.
%
%We show that in such a scenario, the coded caching gain can be increased interestingly by a multiplicative factor proportional to the receiver antenna count. In other words, if every user has $G$ receiving antennas and $\frac{L}{G}$ is an integer, we propose a novel coded caching scheme where with every single transmission, it is possible to send $Gt + L$ independent streams to the users. 
%
%The key to achieving this multiplicative improvement in caching gain is in the use of signal-level interference cancellation approach similar to the one presented in~\cite{lampiris2018adding}, as well as a shared-cache user grouping mechanism similar to that presented in~\cite{salehi2020lowcomplexity} for enabling extremely low subpacketization requirement. In this extended abstract, we introduce the general procedure and clarify the idea with a small example. A more detailed explanation will be provided in the extended version of the paper. To the best of our knowledge, this work is the first one to present the possibility of such an improved \ac{DoF} gain in cache-aided \ac{MIMO} communications.
%
%In a nutshell, the elevation algorithm works as follows: for a given $K$-user \ac{MIMO} network with $L$ antennas at the transmitter and more than $G$ antennas at each receiver, %\footnote{In fact, $L$ and $G$ represent the maximum number of independent streams at the transmitter and receivers, respectively. For simplicity, here we assume the number of independent streams is equal to the number of antennas, i.e., the channel matrix from the transmitter to each receiver is full-rank. Moreover, we also assume the RX processing is antenna-specific (i.e. no beamforming is done at the receiver side).} 
%we first consider a virtual \ac{MISO} network with the same number of $K$ users and caching gain $t$, but with $\eta$ antennas at the transmitter. Then, we design cache placement and transmission vectors for the virtual network following one of the available linear \ac{MISO} schemes in the literature (the baseline scheme should support signal-level interference cancellation as explained later on). Finally, cache contents for users in the real network are set to be the same as in the virtual network, and the transmission vectors are \textit{stretched} to support multi-antenna receivers and increased \ac{DoF}. In this extended abstract, we clarify the procedure using an example, and leave the detailed explanation for the extended version of the paper. %For clarification, here we review these three steps for a small, example network.

%Before proceeding with the example, let us define some notations. For any integer $J$, we use $[J]$ to denote the set of numbers $\{1,2,...,J\}$. The set of users is shown by $\CK$. A general file in the library is shown by $W$, and the file requested by user $u_k \in \CK$ is denoted by $W(k)$. Zero-forcing transmit beamformer vectors for real and virtual networks are denoted by $\Bw_{\CR}$ and $\hat{\Bw}_{\CR}$, respectively, where the set $\CR$ includes the indices of the user specific streams at which the data is nulled-out by the beamformer. For notation simplicity, we remove the brackets while explicitly writing the stream indices in $\CR$. We also use $\Sfs_k^g$, $g \in [G]$, to refer to stream $g$ intended for user $u_k$. %Finally, the bit-wise XOR operation is denoted by $\oplus$.
%Finally, for two sets $\CA$ and $\CB$, $\CA \backslash \CB$ denotes the set of elements in $\CA$ that are not in $\CB$.

Now, assume a small network with $K=6$ users and caching gain $t=1$, where the transmitter has $L=4$ and every receiver has two antennas.
% at the transmitter, and $G=2$ antennas at each receiver. 
%The coded caching gain is given as $t=1$. 
Using \ac{MISO} schemes, the maximum achievable \ac{DoF} for this network is $L+t = 5$ (multiple receive antennas can be used for additional beamforming gain). However, with the proposed elevation algorithm, the \ac{DoF} value can be increased to $Gt+L=6$, assuming $G=2$ parallel streams for each user are supportable by the channel conditions. Without loss of generality, let us assume the reduced-subpacketization scheme in~\cite{salehi2020lowcomplexity} is chosen as the baseline \ac{MISO} scheme.
%
%Using the original coded caching scheme in~\cite{shariatpanahi2018physical}, the maximum achievable \ac{DoF} for this network would be $L+t = 5$. Note that with this scheme, multiple antennas at the receivers are used only to improve the \ac{SINR}. However, we show that with the new scheme, it is possible to serve $Gt+L =6$ independent data streams with every single transmission (i.e., the achievable \ac{DoF} is increased to 6). 
The first step is to find proper parameters for the virtual \ac{MISO} network. Clearly, the virtual network has the same number of $K=6$ users and caching gain $t=1$, but with $\eta = 2$ antennas at the transmitter and one antenna at each receiver. Cache placement in the virtual network directly follows that of~\cite{salehi2020lowcomplexity}, i.e., every file $W$ is first split into $K=6$ equal-sized \textit{packets} denoted by $W_p$, $p \in [6]$, and then, each packet is split into $t+\eta=3$ smaller \textit{subpackets} denoted by $W_p^q$, $q \in [3]$. Finally, in the cache memory of user $u_k$, we store $W_k^q$, for every $W$ and $q$. 

%For simplicity, we use the tabular view in Figure~\ref{fig:Graphical_base} to represent the cache placement in this network. In this representation, a darkly shaded cell in row $p$ and column $k$ denotes that the file parts $W_p^q$ for every $W$, $q$ are stored in the cache memory of user $u_k$.

%\input{Figs/GraphicalBase}
\input{Figs/Trans_comp_virtual}

For notational simplicity, let us assume $W(1) \equiv A$, $W(2) \equiv B$, ..., and $W(6) \equiv F$ (note that it is possible for some users to request the same file). Using the coded caching scheme in~\cite{salehi2020lowcomplexity} for the virtual network, the first and second transmission vectors (corresponding to the transmissions in the first and second time intervals) are built as\footnote{Note that virtual beamformer vectors $\hat{\Bw}_{\CR}$ are defined only to clarify the transmission (and decoding) process in the virtual network. We do not need to calculate them at any step.}
\begin{equation}
\label{eq:trans_vector_exmp_virtual}
\begin{aligned}
    \hat{\Bx}_1 &= A_2^1 \hat{\Bw}_3 + B_1^1 \hat{\Bw}_3 + C_1^1 \hat{\Bw}_2 , \\
    \hat{\Bx}_2 &= A_3^1 \hat{\Bw}_4 + C_1^2 \hat{\Bw}_4 + D_1^1 \hat{\Bw}_3 .
\end{aligned}
\end{equation}
%where $\Bx_1$ and $\Bx_2$ deliver parts of the requested data to user sets $\{u_1,u_2,u_3\}$ and $\{u_1,u_3,u_4\}$, respectively.
For better clarification, a graphical representation for $\hat{\Bx}_1$ and $\hat{\Bx}_2$ is provided in Figure~\ref{fig:subhatnoxor}. This representation follows the same principles as in~\cite{salehi2020lowcomplexity}, i.e., 
%
%Following the same representation as in~\cite{salehi2020lowcomplexity}, a graphical view of $\Bx_1$ and $\Bx_2$ are shown in Figure~\ref{fig:subhatnoxor}. In graphical representations, 
a black cell means (every subpacket of) the respective data part is available in the cache memory, and a gray cell indicates that (a subpacket of) the respective part is sent during the transmission. 


%Without loss of generality, let us consider the decoding process for $\Bx_1$. As we have used zero-forcing beamformers, after this transmission, users $u_1$, $u_2$ and $u_3$ receive
%\begin{equation}
%    \begin{aligned}
%        y_1(1) &= A_2^1 \Bh_1^H \Bw_3 + B_1^1 \Bh_1^H \Bw_3 + C_1^1 \Bh_1^H \Bw_2 + z_1(1) , \\
%        y_1(2) &= A_2^1 \Bh_2^H \Bw_3 + B_1^1 \Bh_2^H \Bw_3 + z_1(2) , \\
%        y_1(3) &= C_1^1 \Bh_3^H \Bw_2 + z_1(3) , \\
        %y_2(1) &= (A_2^2 \oplus B_1^2) \Bh_1^H \Bw_3 + (A_4^1 \oplus D_1^1) \Bh_1^H \Bw_2 + z_2(1) , \\
%    \end{aligned}
%\end{equation}
%where $\Bh_k$ denotes the (virtual) channel vector for $u_k$,\footnote{The channel vectors here are defined only to explain the decoding process with the signal-level interference cancellation approach within the virtual \ac{MISO} network. They do not have a physical interpretation.} and $z_1(k)$ represents the \ac{AWGN} at the receiver of $u_k$ during the transmission of $\Bx_1$.
%With $y_1(1)$ at its receiver, user $u_1$ first reconstructs $B_1^1 \Bh_1^H \Bw_3$ and $C_1^1 \Bh_1^H \Bw_2$ using its cache contents\footnote{We assume the equivalent channels $\Bh_1^H \Bw_3$ and $\Bh_1^H \Bw_2$ can be (ideally) estimated from the stream specific demodulation pilots [REF].} and removes them from $y_1(1)$, and then, decodes $A_2^1$ interference-free. Similarly, users $u_2$ and $u_3$ also remove the remaining interference using their cache contents and decode (parts of) their requested data interference-free.
%As the remaining interference is here removed with the help of cache contents \textit{before} decoding data, we call this approach \textit{signal-level} interference cancellation. In contrast, in the \textit{bit-level} approach, the interference is removed \textit{after} the decoding is completed. A good example of the bit-level approach can be found in the original \ac{MISO} scheme in~\cite{shariatpanahi2018physical}, where the cache-aided interference removal (with XOR operation) is done after decoding the codewords.\footnote{It should be noted that the bit-level approach in~\cite{shariatpanahi2018physical} can be easily transformed to the signal-level approach by avoiding the XOR operation inside codewords and using a separate beamformer vector for each data packet. As a result, the proposed elevation scheme can also be applied to the coded caching scheme in~\cite{shariatpanahi2018physical}, but with an additional step. This is explained in more detail in the extended version of the paper.}

%first decodes $(A_2^1 \oplus B_1^1)$ and $(A_3^1 \oplus C_1^1)$ using a \ac{SIC} receiver, and then uses its cache contents to remove $B_1^1$ and $C_1^1$ to get $A_2^1$ and $A_3^1$ interference-free. As the cache contents are used after the decoding process, this procedure is called the bit-level interference cancellation approach. 
%From a different perspective, we can built this transmission vector as
%\begin{equation}
%\begin{aligned}
%\label{eq:trans_vector_exmp_signal_level_virtual}
%    \Bar{\Bx}_1 = A_2^1 \Bw_3 + B_1^1 \Bar{\Bw}_3 + A_3^1 \Bw_2 + C_1^1 \Bar{\Bw}_2 + B_3^1 \Bw_1 + C_2^1 \Bar{\Bw_1},
%\end{aligned}
%\end{equation}
%where the bars are used only to distinguish various beamforming vectors that zero-force data at the same subset of users. With this approach, $u_1$ receives
%\begin{equation}
%\begin{aligned}
%    \Bar{y}_1(1) = &A_2^1 \Bh_1^H \Bw_3 + B_1^1 \Bh_1^H \Bar{\Bw}_3 \\
%    &+ A_3^1 \Bh_1^H \Bw_2 + C_1^1 \Bh_1^H \Bar{\Bw_2} + z_1(1) ,
%\end{aligned}
%\end{equation}
%and has to reconstruct and remove the interference terms $B_1^1 \Bh_1^H \Bar{\Bw}_3$ and $C_1^1 \Bh_1^H \Bar{\Bw}_2$ using its cache contents, before using a \ac{SIC} receiver (for getting $A_2^1$ and $A_3^1$ interference-free). As the interference is now removed before decoding the received signal, this approach is called signal-level interference cancellation. 

%Note that using the same signal-level approach, without any \ac{DoF} loss, we can also use the following two transmissions instead of $\Bar{\Bx}_1$ to avoid the SIC receiver
%\begin{equation}
%\begin{aligned}
%\label{eq:trans_vector_exmp_signal_level_virtual_decouple}
%    \Bar{\Bx}^1_1 &= A_2^1 \Bw_3 + B_1^1 \Bar{\Bw}_3 + C_1^1 \Bar{\Bw}_2  \\
%    \Bar{\Bx}^2_1 &= A_3^1 \Bw_2 + B_3^1 \Bw_1 + C_2^1 \Bar{\Bw}_1.
%\end{aligned}
%\end{equation}
%In other words, without any \ac{DoF} loss, we can use more transmissions to avoid \ac{SIC} receivers (this approach is similar to controlling the multiple access channel size with the $\beta$ parameter in~\cite{tolli2017multi}). In this paper, for its simplicity, we use this model to explain our new scheme for the increased \ac{DoF} (note that it is also possible to use the \ac{SIC}-requiring approach as in~\eqref{eq:trans_vector_exmp_signal_level_virtual}, and this selection is only made to make the explanation simpler). 

%Moreover, we also use a simple graphical representation to show how various transmission vectors are formed. In Figure~\ref{fig:Graphical_base}, we have provided the graphical representation for both bit- and signal-level transmission vectors $\Bx_1$ and $\Bar{\Bx}_1$, as presented in~\eqref{eq:trans_vector_exmp_bit_level} and~\eqref{eq:trans_vector_exmp_signal_level_virtual}, respectively. In this figure, darkly shaded cells represent cached data parts at different users, while lightly shaded ones denote the parts being transmitted with the transmission vectors. Similarly, in Figure~\ref{fig:subhatnoxor}, we have provided the graphical representation for \ac{SIC}-avoiding signal-level transmission vectors $\Bar{\Bx}_1^1$ and $\Bar{\Bx}_1^2$ as presented in~\eqref{eq:trans_vector_exmp_signal_level_virtual_decouple}.


%The graphical representation for these two approaches is provided in Figure~\ref{fig:subhatnoxor}, where the lightly shaded cells represent the file parts being sent during each transmission.

%\input{Figs/GraphicalBase}

Now, transmission vectors for the original \ac{MIMO} setup can be found by stretching the transmission vectors in~\eqref{eq:trans_vector_exmp_virtual}. For stretching, for every term $W_p^q(k) \hat{\Bw}_{\CR}$ in a transmission vector of the virtual network, we 
%
%Using the decoupled version as in~\eqref{eq:trans_vector_exmp_signal_level_virtual_decouple} for the virtual network, we can \textit{elevate} the transmission vectors to support the extended \ac{DoF} in the original network. 
%
%The procedure is as follows: 
first split $W_p^q(k)$ into $G$ smaller parts $W_p^{q,g} (k)$, $g \in [G]$, and then replace the whole term with
\begin{equation}
    W_p^q(k) \hat{\Bw}_{\CR} \; \rightarrow \; W_p^{q,1} (k) \Bw_{\CR_1} +  ... + W_p^{q,G} (k) \Bw_{\CR_G} ,
\end{equation}
where the new zero-forcing sets $\CR_g$ are built as
\begin{equation}
    \CR_g = \bigcup_{u_{\Bar{k}} \in \CR} \{ \Sfs_{\Bar{k}}^1, ... , \Sfs_{\Bar{k}}^G \} \; \cup \; \{ \Sfs_k^1, ... , \Sfs_k^G \} \backslash \{ \Sfs_k^g \} .
\end{equation}
In other words, instead of a data stream $W_p^q(k)$ for user $u_k$, we consider $G$ parallel streams $W_p^{q,g}(k)$, where each stream will be assigned distinct receive beamformer at user $u_k$. Moreover, if the zero-forcing set for $W_p^q (k)$ is $\CR$, the zero-forcing set for $W_p^{q,g}(k)$ includes every dedicated stream for every user in $\CR$, as well as $G-1$ streams for $u_k$ (i.e., every stream for $u_k$ except $\Sfs_k^g$). This means $W_p^{q,g}(k)$ must be zero-forced at a total number of
\begin{equation}
    (\eta-1)G + G-1 = \eta G -1 = L-1 
\end{equation}
locations (i.e, streams), which is indeed possible as we have $L$ antennas at the transmitter. For the example network, the stretched version of $\hat{\Bx}_1$ can be written as
\begin{equation}
\begin{aligned}
    {\Bx}_1 =& A_2^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + A_2^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} \\
    & + B_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
    & + C_1^{1,1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1} ,
\end{aligned}
\end{equation}
and for $\hat{\Bx}_2$ we can write
\begin{equation}
\begin{aligned}
    {\Bx}_2 =& A_3^{1,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^2} + A_3^{1,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^1} \\
    & + C_1^{2,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^2} + C_1^{2,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^1} \\
    & + D_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^2} + D_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^1} .
\end{aligned}
\end{equation}
Note that in this example, zero-forcing at three locations is possible as the number of transmitter antennas is given as $L=4$. The graphical representations for these transmissions are provided in Figures~\ref{fig:extended} and~\ref{fig:extended_second}. As can be seen, they seem like the stretched versions of the base representations provided in Figure~\ref{fig:subhatnoxor}, and hence, we use the term \textit{stretching} to denote the proposed set of operations.

\input{Figs/Trans_extended_first_trans}

\input{Figs/Trans_extended_second}

For clarification, let us review the decoding process for each stream of user $u_1$ in ${\Bx}_1$. As we have used zero-forcing beamformers, the received signal vector at user $u_1$ is 
\begin{equation}
    \begin{aligned}
        \By_1 = \BH_1 {\Bx}_1 + \Bz_1=& A_2^{1,1} \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + \BI_1 +  \Bz_1 ,
    \end{aligned}
\end{equation}
where $\BH_{1} \in \mathbb{C}^{2 \times 4}$ denotes the channel matrix between user $1$ and the transmitter, $\Bz_1$ represents the \ac{AWGN} vector at $u_1$ during the transmission of $\Bx_1$, and $\BI_1$ denotes the interference term. Now, the stream-specific received signal for $\Sfs_1^1$ can be written as
\begin{equation}
    \begin{aligned}
        y_1(\Sfs_1^1) := \Bu_{\Sfs_1^1}^H \By_1 =& A_2^{1,1} \Bu_{\Sfs_1^1}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + I_1(\Sfs_1^1) +  z_1(\Sfs_1^1) ,
    \end{aligned}
\end{equation}
where $\Bu_{\Sfs_1^1} \in \mathbb{C}^{2}$ denotes the dedicated receive beamformer for stream $\Sfs_1^1$ at user $1$ and $z_1(\Sfs_1^1)$ represents its corresponding noise. The interference term $I_1(\Sfs_1^1)$ is defined as
\begin{equation}
    \begin{aligned}
        I_1(\Sfs_1^1) := & + B_1^{1,1} \Bu_{\Sfs_1^1}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
        & + C_1^{1,1} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1}.
    \end{aligned}
\end{equation}
However, the user $u_1$ has $B_1^1$ and $C_1^1$ in its cache memory, and hence, it can reconstruct and remove the whole interference term $I_1(\Sfs_1^1)$ from $y_1(\Sfs_1^1)$,\footnote{We assume the term ($\Bu_{\Sfs^{g}_{{k}}}^{H} \BH_{k} \Bw_{\CR}$) can be estimated from stream-specific demodulation pilots.} to decode $A_2^{1,1}$ interference-free. Similarly, the stream-spicific received signal for $\Sfs_1^2$ of user $u_1$ is
\begin{equation}
    \begin{aligned}
        y_1(\Sfs_1^2) :=\Bu_{\Sfs_1^2}^H \By_1 =& A_2^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} + I_1(\Sfs_1^2) +  z_1(\Sfs_1^2) ,
    \end{aligned}
\end{equation}
where $\Bu_{\Sfs_1^2} \in \mathbb{C}^{2}$ denotes the dedicated receive beamformer for stream $\Sfs_1^2$ at user $1$ and the interference term $I_1(\Sfs_1^2)$ is defined as
\begin{equation}
    \begin{aligned}
        I_1(\Sfs_1^2) := & + B_1^{1,1} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
        & + C_1^{1,1} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1}.
    \end{aligned}
\end{equation}
Again, the user $u_1$ can reconstruct and remove the interference term $I_1(\Sfs_1^2)$ using its cache contents, and decode $A_2^{1,2}$ interference-free. Following the same procedure for users $u_2$ and $u_3$, each of them can decode two parallel streams after the transmission of $\Bx_1$, and hence, the increased \ac{DoF} value of $6$ can be achieved for the considered \ac{MIMO} setup. It should be noted that, as the remaining interference is here removed with the help of cache contents \textit{before} decoding data, we call this approach \textit{signal-level} interference cancellation. In contrast, in the \textit{bit-level} approach, the interference is removed \textit{after} the decoding is completed. A good example of the bit-level approach can be found in the original \ac{MISO} scheme in~\cite{shariatpanahi2018physical}, where the cache-aided interference removal (with XOR operation) is done after decoding the codewords. However, the bit-level approach in~\cite{shariatpanahi2018physical} can be easily transformed to the signal-level approach by avoiding the XOR operation inside codewords and using a separate beamformer vector for each data packet. As a result, the proposed elevation algorithm can also be applied to the coded caching scheme in~\cite{shariatpanahi2018physical}, but with an additional step. This is explained in more detail in the extended version of the paper.

In summary, our new scheme enables $t+\eta$ users to be served with each transmission, and delivers $G$ independent streams to each of these users. This results in a total number of $G(t+\eta) = Gt+L$ independent streams, and hence, a multiplication in the coded caching gain $t$ compared to the state-of-art. %To the best of our knowledge, this is the first scheme to show such a multiplicative increase in the coded caching gain is possible in cache-enabled \ac{MIMO} setups.
If the baseline \ac{MISO} scheme is chosen as the one in~\cite{salehi2020lowcomplexity},
the total subpacketization requirement for the elevated \ac{MIMO} scheme is
\begin{equation}
    G K (t + \eta) = K(Gt + L)
    %G \binom{K}{t} \binom{K-t-1}{\eta - 1}.
\end{equation}
In the extended version of this paper, we present a detailed explanation of the proposed method, and thoroughly investigate the possibility of using other baseline \ac{MISO} schemes. We also relax the antenna-specific RX processing assumption by considering stream-specific processing, and compare our algorithm with the state-of-art from the achievable \ac{DoF} and subpacketization requirement perspectives.
%A detailed explanation of the proposed method, the possibility of using other baseline \ac{MISO} schemes, and more comparisons with the state-of-art from the achievable \ac{DoF} and subpacketization requirement perspectives are due for the extended version of this paper.

%The text needs a major revision:
%\begin{enumerate}
%    \item The literature review part should be updated to include works by Petros and Emanuele on shared cache settings~\cite{parrinello2019fundamental,parrinello2020extending}.
%    \item Our contribution should be clarified: we consider a MIMO system and based on the previous results from Emanuele and Petros, show that multiple receiving antennas boost the coded caching gain with a multiplicative factor.
%    \item Then, we provide a simple extension scheme, that can be applied to any based MISO scheme, which achieves the full enhanced coded caching gain in the MIMO setup.
%    \item We show that by using this extension on top of the base scheme in the TWC work, we can have a linear (or quadratic) subpacketization increase while achieving the full enhanced caching gain.
%    \item The example should be updated accordingly; it should reflect transmission vectors built with the TWC scheme instead of MS.
%\end{enumerate}

==> Figs/data.tex <==
SNR	LG2WSA	LG2Prop	LG2Virt	LG3WSA	LG3Prop	LG3Virt	LG4WSA	LG4Prop	LG4Virt
0	0.37888793	0.478117902	0.466257565	0.593597422	0.780987656	0.711628686	0.800458582	1.06431067	0.961240276
5	0.729799155	0.880695207	0.831109606	1.118585984	1.41256128	1.213001181	1.497419721	1.920078217	1.580935968
10	1.219829283	1.442125356	1.306486601	1.874280467	2.261337182	1.874459492	2.504779923	3.07112509	2.380875754
15	1.865168075	2.148772492	1.898581016	2.823484879	3.2908021	2.690004668	3.789231123	4.466875915	3.371284399
20	2.6516918	2.968059461	2.582472719	3.972802442	4.491072009	3.612707929	5.298912825	6.055180408	4.517150415
25	3.524027859	3.854438097	3.315887094	5.24532053	5.78857596	4.587645251	6.987312257	7.785024556	5.749767519
30	4.43827704	4.764082815	4.067829559	6.382671709	6.920325654	5.5791508	8.785198923	9.598013725	7.01136475
35	5.365618585	5.667276382	4.820442815	7.996043212	8.542984004	6.564780279	10.67738972	11.47607729	8.27289382
40	6.288618404	6.523678995	5.563734365	9.077606483	9.570988372	7.537334729	12.56242257	13.34920575	9.506236754


==> MIMOCC.tex <==
\subsection{The Elevation Procedure}
\label{section:stretching_algorithm}
As stated earlier, our new algorithm for \ac{MIMO} coded caching works through elevation of a baseline signal-level \ac{MISO} scheme.
In a nutshell, this elevation procedure works as follows: for a given $K$-user \ac{MIMO} network with coded caching gain $t$ and spatial multiplexing gains of $L$ and $G$ at the transmitter and receivers, %\footnote{In fact, $L$ and $G$ represent the maximum number of independent streams at the transmitter and receivers, respectively. For simplicity, here we assume the number of independent streams is equal to the number of antennas, i.e., the channel matrix from the transmitter to each receiver is full-rank. Moreover, we also assume the RX processing is antenna-specific (i.e. no beamforming is done at the receiver side).} 
we first consider a virtual \ac{MISO} network with the same number of $K$ users and caching gain $t$, but with the spatial multiplexing gain of $\eta = \frac{L}{G}$ at the transmitter. Then, we design cache placement and transmission vectors for the virtual network following one of the available signal-level \ac{MISO} schemes in the literature. Finally, cache contents for users in the real network are set to be the same as the virtual network, but transmission vectors of the virtual network are \textit{stretched} to support multi-stream receivers and the increased \ac{DoF}. %In this extended abstract, we clarify the procedure using an example, and leave the detailed explanation for the extended version of the paper. 

%Now, transmission vectors for the original \ac{MIMO} setup can be found by stretching the transmission vectors in~\eqref{eq:trans_vector_exmp_virtual}. 
The stretching process of the transmission vectors of the virtual network is straightforward. Assume the zero-forcing beamformers for the virtual network are shown with $\Bw_{\CT}$, where $\CT$ denotes the set of users where the data is zero-forced.\footnote{Note that the virtual network has a \ac{MISO} setup, and hence, each user can receive only one data stream at a time. Moreover, virtual beamformer vectors $\Bw_{\CT}$ are defined only to clarify the transmission (and decoding) process in the virtual network, and hence, it is not necessary to calculate their exact values at any step.} Then, a transmission vector $\hat{\Bx}$ of the virtual network is a linear combination of $t+\eta$ terms $W_p^q(k) \Bw_{\CT(k)}$, where $W_p^q(k)$ denotes a subpacket of the file $W(k)$ requested by user $k$ (the subpacket index is clarified by $p$ and $q$), and $\Bw_{\CT(k)}$ is the beamformer vector associated with $W_p^q(k)$. Now, for stretching, for every term $W_p^q(k) \Bw_{\CT(k)}$ in $\hat{\Bx}$, we
%For every term $W_p^q(k) \Bv_{\CT}$ in a transmission vector $\hat{\Bx}$ of the virtual network, we 
%
%Using the decoupled version as in~\eqref{eq:trans_vector_exmp_signal_level_virtual_decouple} for the virtual network, we can \textit{elevate} the transmission vectors to support the extended \ac{DoF} in the original network. 
%
%The procedure is as follows: 
first split the subpacket $W_p^q(k)$ into $G$ smaller parts $W_p^{q,g} (k)$, $g \in [G]$, and then replace the term with
\begin{equation}
\label{eq:stretch_main}
    W_p^q(k) \Bw_{\CT(k)} \; \rightarrow \; W_p^{q,1} (k) \Bw_{\CR_1} +  \cdot \cdot \cdot + W_p^{q,G} (k) \Bw_{\CR_G} ,
\end{equation}
where the zero-forcing sets $\CR_g$ for the real \ac{MIMO} network are built as
\begin{equation}
\label{eq:stretch_zfset}
    \CR_g = \bigcup_{\Bar{k} \in \CT(k)} \{ \Sfs_{\Bar{k}}^1, \cdot \cdot \cdot , \Sfs_{\Bar{k}}^G \} \; \cup \; \{ \Sfs_k^1, \cdot \cdot \cdot , \Sfs_k^G \} \backslash \{ \Sfs_k^g \} .
\end{equation}
In other words, instead of a single data stream $W_p^q(k)$ for user $k$ in the virtual network, we consider $G$ parallel streams $W_p^{q,g}(k)$ for user $k$ in the real network. Moreover, if the zero-forcing set for $W_p^q (k)$ in the virtual network is $\CT(k)$, the interference from $W_p^{q,g}(k)$ in the real network should be zero-forced at:
\begin{enumerate}
    \item Every stream sent to every user $\Bar{k} \in \CT(k)$. As $|\CT(k)| = \eta-1$ and each stream in the virtual network is transformed into $G$ streams in the real network, this includes $G \times (\eta-1)$ streams in total;
    \item Every other stream sent to user $k$. This includes $G-1$ streams in total.
\end{enumerate}
As a result, the interference from $W_p^{q,g}(k)$ must be zero-forced on a total number of
\begin{equation}
    G (\eta-1) + G-1 = \eta G -1 = L-1 
\end{equation}
streams in the real network, which is indeed possible as the spatial multiplexing gain of $L$ is achievable at the transmitter. In the following subsection, we review the elevation procedure using a simple example network. We also discuss how the received signal is decoded by the users.

%-------------------------------------------------------------------------------%
\subsection{A Clarifying Example}
Let us consider a small network with $K=6$ users and caching gain $t=1$, where the spatial multiplexing gains of $L=4$ and $G=2$ are achievable at the transmitter and receivers, respectively.
% at the transmitter, and $G=2$ antennas at each receiver. 
%The coded caching gain is given as $t=1$. 
Using \ac{MISO} schemes, the maximum achievable \ac{DoF} for this network is $L+t = 5$.\footnote{Note that in this case, multiple receive antennas can be used for achieving an additional beamforming gain (cf.~\cite{tolli2017multi}). However, they do not result in any increase in the \ac{DoF} value.} However, with the proposed elevation algorithm, the achievable \ac{DoF} can be increased to $Gt+L=6$. As mentioned earlier, without any loss of generality, we assume the reduced-subpacketization scheme in~\cite{salehi2020lowcomplexity} is chosen as the baseline \ac{MISO} scheme.

The first step is to find proper parameters for the virtual \ac{MISO} network. Clearly, the virtual network has the same number of $K=6$ users and caching gain $t=1$, but the spatial multiplexing gain of $\eta = \frac{L}{G} = 2$ at the transmitter. Cache placement in the virtual network directly follows that of~\cite{salehi2020lowcomplexity}, i.e., every file $W \in \CF$ is first split into $K=6$ equal-sized \textit{packets} denoted by $W_p$, $p \in [6]$, and then, each packet is split into $t+\eta=3$ smaller \textit{subpackets} denoted by $W_p^q$, $q \in [3]$. Finally, every user $k$ caches $W_k^q$, for every $W \in \CF$ and $q \in [3]$. For example, user one caches $\{W_1^1, W_1^2, W_1^3 \}$, for every file $W$ in the library.

\input{Figs/Trans_comp_virtual}

For simplicity, let us use $W(1) \equiv A$, $W(2) \equiv B$, ..., and $W(6) \equiv F$ (note that it is still possible for some users to request the same file). Using the coded caching scheme in~\cite{salehi2020lowcomplexity} for the virtual network, the first and second transmission vectors (corresponding to the transmissions in the first and second time intervals) are built as
\begin{equation}
\label{eq:trans_vector_exmp_virtual}
\begin{aligned}
    \hat{\Bx}(1) &= A_2^1 \Bw_{3} + B_1^1 \Bw_3 + C_1^1 \Bw_2 , \\
    \hat{\Bx}(2) &= A_3^1 \Bw_4 + C_1^2 \Bw_4 + D_1^1 \Bw_3 ,
\end{aligned}
\end{equation}
where the brackets for the zero-forcing sets are ignored for notational simplicity.
%where $\Bx_1$ and $\Bx_2$ deliver parts of the requested data to user sets $\{u_1,u_2,u_3\}$ and $\{u_1,u_3,u_4\}$, respectively.
For better clarification, graphical representations for $\hat{\Bx}(1)$ and $\hat{\Bx}(2)$ are provided in Figure~\ref{fig:subhatnoxor}. These representations follow the same principles as in~\cite{salehi2020lowcomplexity}, i.e., 
%
%Following the same representation as in~\cite{salehi2020lowcomplexity}, a graphical view of $\Bx_1$ and $\Bx_2$ are shown in Figure~\ref{fig:subhatnoxor}. In graphical representations, 
a black cell means (every subpacket of) the respective data part is available in the cache memory, and a gray cell indicates that (a subpacket of) the respective part is sent during the transmission. 

Now, using the stretching mechanism in~\eqref{eq:stretch_main},  the stretched version of $\hat{\Bx}(1)$ can be written as
\begin{equation}
\begin{aligned}
    {\Bx}(1) =& A_2^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + A_2^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} \\
    & + B_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
    & + C_1^{1,1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1} ,
\end{aligned}
\end{equation}
where the brackets for the zero-forcing sets are ignored for notational simplicity. Similarly, for $\hat{\Bx}(2)$ we can write
\begin{equation}
\begin{aligned}
    {\Bx}(2) =& A_3^{1,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^2} + A_3^{1,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^1} \\
    & + C_1^{2,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^2} + C_1^{2,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^1} \\
    & + D_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^2} + D_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^1} .
\end{aligned}
\end{equation}
Note that in this example, zero-forcing the interference of one data stream on three other streams is possible as the spatial multiplexing gain of $L=4$ is achievable at the transmitter. The graphical representations for these transmissions are provided in Figures~\ref{fig:extended} and~\ref{fig:extended_second}. As can be seen, they seem like the stretched versions of the base representations provided in Figure~\ref{fig:subhatnoxor}, and hence, we use the term \textit{stretching} to denote the proposed set of operations.

\input{Figs/Trans_extended_first_trans}

\input{Figs/Trans_extended_second}

Now, let us review the decoding process for each stream of user one as ${\Bx}(1)$ is transmitted. The received signal at this user can be written in the vector form as 
\begin{equation}
    \begin{aligned}
        \By_1(1) &= \BH_1 {\Bx}(1) + \Bz_1(1) \\
        &= A_2^{1,1} \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + A_2^{1,2} \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} \\
        &\qquad+ \BH_1 \BI_1(1) +  \Bz_1(1) ,
    \end{aligned}
\end{equation}
where $\BI_1(i)$ is the interference term at user one at the first time interval, defined as
\begin{equation}
    \begin{aligned}
        \BI_1(1) &= B_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
        & + C_1^{1,1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1} .
    \end{aligned}
\end{equation}
The next step is to multiply the received signal $\By_1(1)$ by receive beamformers $\Bu_{1,1}$ and $\Bu_{1,2}$, in order to extract $\Sfs_1^1$ and $\Sfs_1^2$, respectively. After multiplication by $\Bu_{1,1}$ we get
\begin{equation}
    \begin{aligned}
        y_1^1(1) &= \Bu_{1,1}^H \By_1(1) = \Bh_{1,1}^H \Bx(1) + z_{1,1}(1) \\
        &= A_2^{1,1} \Bh_{1,1}^H \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + \Bh_{1,1}^H \BI_1(1) +  z_{1,1}(1) \; ,
    \end{aligned}
\end{equation}
where $\Bh_{1,1}$ and $z_{1,1}(1)$ are the equivalent channel vector and \ac{AWGN} for the first stream of user one during this transmission as defined in Section~\ref{section:sys_model}, and we have used the zero-force beamforming property
\begin{equation}
    \Bh_{1,1}^H \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} = 0 \; .
\end{equation}
However, user one has all the terms $B_1^{1,1}$, $B_1^{1,2}$, $C_1^{1,1}$, and $C_1^{1,2}$ in its cache memory. Hence, with the equivalent channel multiplier knowledge, it can build and remove the interference term $\Bh_{1,1}^H \BI_1(1)$ from $y_1^1(1)$, to decode the requested term $A_1^{1,1}$ interference-free. Similarly, multiplying by $\Bu_{1,2}$ results in
\begin{equation}
    \begin{aligned}
        y_1^2(1) &= \Bu_{1,2}^H \By_1(1) = \Bh_{1,2}^H \Bx(1) + z_{1,2}(1) \\
        &= A_2^{1,2} \Bh_{1,2}^H \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} + \Bh_{1,2}^H \BI_1(1) +  z_{1,2}(1) \; .
    \end{aligned}
\end{equation}
Again, user one can use its cache contents and the acquired equivalent channel multipliers to build and remove $\Bh_{1,2}^H \BI_1(1)$ from $y_1^2(1)$, and decode $A_1^{1,2}$ interference-free. As a result, user one receives two parallel data streams from the transmission of $\Bx(1)$. Similarly, users two and three each receive two parallel data streams, and hence, a total number of six data streams are delivered to the users during the first time interval. The same procedure is repeated during every transmission, and the increased \ac{DoF} of $Gt+L = 6$ becomes possible. Note that here, the cache-aided interference cancellation (i.e., removing $\Bh_{1,1}^H \BI_1(1)$ and $\Bh_{1,2}^H \BI_1(1)$) occurs before decoding $y_1^1(1)$ and $y_1^2(1)$, and hence, we have a signal-level coded caching scheme. Moreover, as $p \in [6]$, $q \in [3]$, and $g \in [2]$, the total subpacketization of the caching scheme in this example network is $6 \times 3 \times 2 = 36$.

%------------------------------------------------------------------------------------%
\subsection{Performance and Complexity Analysis}
It can be easily verified that using the proposed elevation mechanism, if the baseline \ac{MISO} scheme achieves \ac{DoF} of $t+L$, the resulting \ac{MIMO} scheme can deliver $Gt+L$ parallel streams to the users during each transmission. This is because for the original network with parameters $K$, $t$, $L$, and $G$, the virtual \ac{MISO} network has the same number of $K$ users and coded caching gain $t$, but the transmitter-side multiplexing gain is reduced to $\eta = \frac{L}{G}$. So, each transmission vector in the virtual network delivers data to $t+\eta$ users simultaneously. However, according to~\eqref{eq:stretch_main}, during the stretching process every data stream in a transmission vector of the virtual network is replaced by $G$ data stream for the real network. So, in every transmission vector for the original \ac{MIMO} network we deliver
\begin{equation}
    G(t+\eta) = Gt + L
\end{equation}
parallel streams, and hence, the \ac{DoF} is increased to $Gt+L$. As discussed in~\cite{parrinello2019fundamental}, this \ac{DoF} value is also optimal among any linear coded caching scheme with uncoded cache placement and single-shot data delivery.

The subpacketization value of the resulting \ac{MIMO} scheme depends on the subpacketization requirement of the baseline \ac{MISO} scheme. If the subpacketization of the baseline scheme is $f(K,t,L)$, where $K$, $t$, and $L$ represent the user count, the coded caching gain, and the transmitter-side multiplexing gain, respectively, the resulting \ac{MIMO} scheme from the proposed elevation mechanism will have the subpacketization of
\begin{equation}
    G \times f(K,t,\eta) \; .
\end{equation}
This is because the subpacketization requirement for the virtual network is $f(K,t,\eta)$, and during the elevation process, each subpacket is further split into $G$ smaller parts. So, for example, if the low-subpacketization scheme in~\cite{salehi2020lowcomplexity} is selected as the baseline \ac{MISO} scheme, the subpacketization requirement would be
\begin{equation}
    G \times K(t+\eta) = K(Gt+L) \; .
\end{equation}
However, the scheme in~\cite{salehi2020lowcomplexity} is applicable to the virtual network only if $\eta \ge t$, or $L \ge Gt$. On the other hand, if we select the original \ac{MISO} scheme in~\cite{shariatpanahi2018multi} as the baseline, the resulting \ac{MIMO} scheme would have the subpacketization requirement of
\begin{equation}
    G \times \binom{K}{t} \binom{K-t-1}{\eta-1} \; ,
\end{equation}
and the scheme would be applicable regardless of $t$, $L$, and $G$ values as long as $\eta$ is an integer. In summary, depending on the selection of the baseline scheme, the resulting \ac{MIMO} scheme can benefit from a very low subpacketization complexity. The subpacketization growth with the user count can even be linear, if the baseline scheme is chosen as the one in~\cite{salehi2020lowcomplexity}.

==> SigLevelIntCan.tex <==
The \ac{MISO} coded caching scheme in~\cite{lampiris2018adding} introduced a novel cache-aided interference cancellation approach, different than~\cite{shariatpanahi2018physical}, to reduce the subpacketization without altering the maximum achievable \ac{DoF}. This approach, which we refer to as the signal-level approach, removes the interference using the cache contents \textit{before} the signal is decoded at the receiver. This is in contrast with the classical bit-level approach, where the cache-aided interference removal is done \textit{after} decoding the received signal. Many other papers in the literature, including the one in~\cite{salehi2020lowcomplexity}, have also used the signal-level approach to reduce the required subpacketization. It is worth mentioning that, although we consider only the subpacketization issue here, the signal-level approach also has other benefits such as enabling much simpler optimized beamformer designs, as demonstrated in~\cite{salehi2020lowcomplexity}.

The \ac{MIMO} coded caching scheme proposed in this paper can be built using any baseline \ac{MISO} scheme with the signal-level interference cancellation approach. Interestingly though, with minor modifications, any bit-level \ac{MISO} coded caching scheme can be transformed into an equivalent signal-level \ac{MISO} scheme, without any DoF loss. The key to this transformation is to decouple the codewords and use a separate beamformer for every data element being sent. The following example enlightens the difference between the signal- and bit-level approaches, and shows how a bit-level scheme can be transformed to an equivalent signal-level scheme.

\begin{exmp}
\label{exmp:sig_bit_level}
Consider a small {MISO} setup with $K=3$ users where the coded caching gain is $t=1$ and the spatial multiplexing gain of $L=2$ can be achieved at the transmitter. Let us consider the bit-level coded caching scheme in~\cite{shariatpanahi2018physical} as the baseline. This scheme requires each file $W \in \CF$ to be split into three subpackets $W_p$, $p \in [3]$. The user $k$, $k \in [3]$, stores subpackets $W_k$ of every file $W$ in its cache memory; i.e., the cache contents of user $k$ are $\{W_k;\;\forall W\in\CF\}$. Then, during the delivery phase, if the files requested by users 1-3 are shown by $A$, $B$, and $C$, respectively, we transmit
\begin{equation}
    \Bx = (A_2 \oplus B_1) \Bw_3 + (A_3 \oplus C_1) \Bw_2 + (B_3 \oplus C_2) \Bw_1 \; ,
\end{equation}
where $\oplus$ represents the bit-wise XOR operation, and $\Bw_k$ is the zero-forcing vector for user $k$ (i.e., $\Bh_k^H \Bw_k = 0$, where $\Bh_k$ is the channel vector from the transmitter to user $k$). Without loss of generality, let us consider the decoding process at user one. Following the zero-force beamforming definition, this user receives
\begin{equation}
    y_1 = (A_2 \oplus B_1) \Bh_1^H \Bw_3 + (A_3 \oplus C_1) \Bh_1^H \Bw_2 + z_1 \; ,
\end{equation}
where $z_1$ represents the \ac{AWGN} at user one. The next step is to decode both $(A_2 \oplus B_1)$ and $(A_3 \oplus C_1)$ from $y_1$, using, for example, a \ac{SIC} receiver. Finally, \emph{after} decoding, user one has to use its cache contents to remove $B_1$ and $C_1$ from the resulting terms, to get $A_2$ and $A_3$ interference-free. As the cache-aided interference cancellation is done after the received signal is decoded at the receiver, we have a bit-level coded caching scheme here. %A graphical representation of this bit-level scheme and the corresponding decoding process in user one is shown in Figure~\ref{fig:subfig_bitlevel}.

In order to transform this scheme into an equivalent signal-level scheme, we need to simply decouple the codewords (i.e., the XOR terms) and use a separate beamformer for every single data element. This means, instead of the transmission vector $\Bx$, we transmit
\begin{equation}
    \Bar{\Bx} = A_2 \Bv_3^1 + B_1 \Bw_3^2 + A_3 \Bw_2^1 + C_1 \Bw_2^2 + B_3 \Bw_1^1 + C_2 \Bw_1^2 \; ,
\end{equation}
where the superscripts are used to distinguish two beamformers with the same zero-forcing set (but different powers). After the transmission of $\Bar{\Bx}$, user one receives
\begin{equation}
    \Bar{y}_1 =  A_2 \Bh_1^T \Bw_3^1 + B_1 \Bh_1^T \Bw_3^2 + A_3 \Bh_1^T \Bw_2^1 + C_1 \Bh_1^T \Bw_2^2 + z_1 \; .
\end{equation}
Then, in order to get its required data elements, i.e., $A_2$ and $A_3$, user one has to first build $B_1 \Bh_1^H \Bw_3^2$ and $C_1 \Bh_1^H \Bw_2^2$ using its cache contents and the acquired channel multiplier information, and remove these interference terms from the received signal \emph{before} decoding it (otherwise, these interference terms will degrade the achievable rate severely). As the cache-aided interference cancellation is now done before the decoding process, this second scheme is using a signal-level approach. %A graphical representation of this signal-level scheme and the corresponding decoding process in user one is shown in Figure~\ref{fig:subfig_siglevel}.
\end{exmp}

\begin{figure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width = \textwidth]{Figs/BitLevelCrop.pdf}
        %\vspace{5pt}
        \caption{Bit-Level Interference Cancellation}
        \label{fig:subfig_bitlevel}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width = \textwidth]{Figs/SignalLevelCrop.pdf}
        \caption{Signal-Level Interference Cancellation}
        \label{fig:subfig_siglevel}
    \end{subfigure}
    \caption{Bit- and Signal-Level Schemes in Example~\ref{exmp:sig_bit_level}}
    \label{fig:bit_sig_level}
\end{figure}

For better clarification, the encoding and decoding processes for the proposed bit- and signal-level schemes in Example~\ref{exmp:sig_bit_level} are shown in Figure~\ref{fig:bit_sig_level}. Note that in this figure, the decoding process for both schemes is shown only for user one. With the same procedure outlined in Example~\ref{exmp:sig_bit_level}, we can transform any \ac{MISO} scheme with the bit-level approach to another one with the signal-level approach. Hence, although our \ac{MIMO} coded caching scheme requires a baseline signal-level \ac{MISO} scheme, this condition does not in fact limit its applicability. Nevertheless, throughout the rest of this paper, we use the scheme in~\cite{salehi2020lowcomplexity}, due to its lower subpacketization, as our baseline scheme.
